Bayes classifier cannot be learned from noisy responses with unknown noise rates

Training a classifier with noisy labels typically requires the learner to specify the distribution of label noise, which is often unknown in practice. Although there have been some recent attempts to relax that requirement, we show that the Bayes decision rule is unidentified in most classification problems with noisy labels. This suggests it is generally not possible to bypass/relax the requirement. In the special cases in which the Bayes decision rule is identified, we develop a simple algorithm to learn the Bayes decision rule, that does not require knowledge of the noise distribution.

==> sections/weighted-erm.tex <==
\section{Weighted ERM in the identifiable case}
\label{sec:weighted-erm}
As we have alluded to before, in the identifiable case (binary classification with $p = (\nicefrac{1}{2}, \nicefrac{1}{2})$) the Bayes decision boundary for clean responses can be consistently estimated by training a classifier with the weighted ERM with any consistent loss. To be concrete, let us consider $\hat f$ as the logit of a classifier that is obtained by minimizing 
\begin{equation}
   \textstyle \frac1n \sum_{i = 1}^n p_n(1 - y_i') \ell(f(x_i), y_i')\,,
\end{equation} where $ p_n(y) = \nicefrac{1}{n} \sum_{i = 1}^n \mathbf{1}\{y'_i = y\}$ and $\ell$ is any  consistent loss function (\ie, if $f^\star$ minimizes the expected risk $\Ex[\ell(f(X), Y)]$ with clean responses then $\mathbbm{1}\{f(x) > 0\}$ is the Bayes classifier). Then $\mathbbm{1}\{\hat f(x) > 0\}$ is a consistent estimator for the Bayes classifier. A reason for such consistency is the following: if the samples are reweighted to make noisy labels class balanced then the Bayes decision boundary for the noisy responses becomes same as the Bayes decision boundary for the clean responses in the original distribution. We formalize the result in the following lemma. 

\begin{lemma}[Reweighted ERM]
\label{lemma:reweighting}
Let $(X, Y, Y') \sim P$ where $Y, Y' \in \{0, 1\}$, $P(Y = 1) = \nicefrac{1}{2}$, the noise rates are instance independent (as in \eqref{eq:ii}), and $\eps_{P}(0, 1) + \eps_P(1, 0) <1$. If the distribution $Q$ is constructed by reweighting $P$ with weights $w(x, y, y') \propto P(Y' = 1-y')$ then the Bayes decision functions for predicting $Y'$ in distribution $Q$ is same as the Bayes decision function for predicting $Y$ in distribution $P$, \ie, 
\begin{equation}
   \big\{x: Q(Y' = 1\mid X = x) \ge  \nicefrac{1}{2} \big\}  = \big\{x: P(Y = 1\mid X = x) \ge  \nicefrac{1}{2} \big\}\,.
\end{equation}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:reweighting}]
Let $w(x, y, y') = c P(Y' = 1-y')$ for some constant $c > 0$. 
According to lemma \ref{lemma:instance-independence-reweighting} with the reweighting  $q(x, y, y') = p(x, y, y') w(x, y,y')$ the instance independence assumption is still valid, \ie, $q(x, y, y') = q(x\mid y) Q(Y = y, Y' = y')$. This means 
\begin{equation}
    \begin{aligned}
    q(x\mid Y = y) Q(Y = y, Y' = y') = p(x\mid Y = y) P(Y = y, Y' = y') c P(Y' = 1-y')\,.
    \end{aligned}
\end{equation} If we integrate both sides with respect to $x$ over the space $\cX$ then we have $\int_{\cX} q(x\mid Y = y) dx = \int_{\cX} p(x\mid Y = y) dx = 1$ and the above equation reduces to 
\begin{equation}
    Q(Y = y, Y' = y') =  P(Y = y, Y' = y') c P(Y' = 1-y')\,.
\end{equation} Now we take a summation over $y$ in the both sides and obtain 
\begin{equation}
    \begin{aligned}
   &\textstyle \sum_{y} Q(Y = y, Y' = y') = \sum_{y} P(Y = y, Y' = y') c P(Y' = 1-y')\\
   \text{or,} ~ & Q(Y' = y') = P(Y' = y') c P(Y' = 1-y') = c p' (1 - p')
    \end{aligned}
\end{equation} where $p' = P(Y' = 1)$. Since, $\sum_{y'}Q(Y' = y') = 1$, from the above equation we obtain $c = \frac{1}{2p'(1 - p')}$ and $w(x, y, y') = \frac1{2 P(Y' = y')}$. 


For $y \in \{0, 1\}$ let us define $\alpha_y (x) = q(x \mid Y' = y') Q(Y' = y')$, $a_y = p(x \mid Y = y) P(Y = y)$, $e_0 = P(Y' = 1\mid Y = 0)$, $e_1 = P(Y' = 0\mid Y = 1)$ and notice that 
\begin{equation} \label{eq:rw.1}
   \begin{aligned}
       \alpha_1 (x) & = q(x \mid Y' = 1) Q(Y' = 1)\\
       & = q(x, 1, 1) + q(x, 0, 1)\\
       & =\textstyle \frac{p(x, 1, 1)}{2 p'} + \frac{p(x, 0, 1)}{2 p'}\\
       & = \textstyle\frac{p(x\mid Y =  1) P(Y = 1)P(Y' = 1\mid Y = 1)}{2 p'}+ \frac{p(x\mid Y =  0) P(Y = 0)P(Y' = 1\mid Y = 0)}{2 p'}\\
       & = \textstyle \frac{a_1(x) \nicefrac{1}{2} (1 - e_1)}{ 2 p'} + \frac{a_0(x) \nicefrac{1}{2} e_0}{ 2 (1- p')} = \frac{a_1(x)  (1 - e_1)}{ 4 p'} + \frac{a_0(x)  e_0}{ 4 p'}\,.
   \end{aligned} 
\end{equation}
Similarly, we obtain 
\begin{equation} \label{eq:rw.2}
    \textstyle \alpha_0(x) = \frac{a_1(x)  e_1}{ 4 (1- p')} + \frac{a_0(x)  (1 - e_0)}{ 4 (1 - p')}\,.
\end{equation} Taking the differences between \eqref{eq:rw.1} and \eqref{eq:rw.2} we obtain 
\begin{equation}
 \textstyle   \alpha_1(x) - \alpha_0(x) = \frac{a_1(x)}{2} \left ( \frac{  1 - e_1}{ 2 p'} - \frac{e_1}{ 2(1 -  p')}\right)  + \frac{a_0(x)}{2} \left( \frac{  e_0}{ 2 p'} - \frac{1 - e_0}{ 2(1 -  p')} \right)\,.
\end{equation} Here, we use 
\begin{equation}
    p' = P(Y' = 1) = \nicefrac{1}{2} (1 - e_1) + \nicefrac{1}{2} e_0  \implies  2p' = 1 - e_1 + e_0,\ ~ \text{and} ~ 2( 1- p') = 1 - e_0 + e_1
\end{equation} in the above equation and obtain 
\begin{equation}
    \begin{aligned}
        \textstyle \alpha_1(x) - \alpha_0(x) & = \textstyle \frac{a_1(x)}{2} \left ( \frac{  1 - e_1}{ 2 p'} - \frac{e_1}{ 2(1 -  p')}\right)  + \frac{a_0(x)}{2} \left( \frac{  e_0}{ 2 p'} - \frac{1 - e_0}{ 2(1 -  p')} \right)\\
        & =\textstyle \frac{a_1(x)}{2} \left ( \frac{  1 - e_1}{ 1 - e_1 + e_0} - \frac{e_1}{ 1 - e_0 + e_1}\right)  + \frac{a_0(x)}{2} \left( \frac{  e_0}{ 1 - e_1 + e_0} - \frac{1 - e_0}{ 1 - e_0 + e_1} \right)\\
        & =\textstyle \frac{a_1(x)}{2} \left ( \frac{  1 - e_1}{ 1 - e_1 + e_0} - \frac{e_1}{ 1 - e_0 + e_1}\right)  + \frac{a_0(x)}{2} \left( 1 - \frac{  1 - e_1}{ 1 - e_1 + e_0} - 1 +  \frac{e_1}{ 1 - e_0 + e_1} \right)\\
        & =\textstyle \frac{a_1(x)}{2} \left ( \frac{  1 - e_1}{ 1 - e_1 + e_0} - \frac{e_1}{ 1 - e_0 + e_1}\right)  + \frac{a_0(x)}{2} \left(  - \frac{  1 - e_1}{ 1 - e_1 + e_0}  +  \frac{e_1}{ 1 - e_0 + e_1} \right)\\
        & =\textstyle \frac{a_1(x) - a_0(x)}{2} \left ( \frac{  1 - e_1}{ 1 - e_1 + e_0} - \frac{e_1}{ 1 - e_0 + e_1}\right)\\
        & = \textstyle \frac{a_1(x) - a_0(x)}{2}  \left ( \frac{1 - e_1 - e_0}{(1 - e_1 + e_0) (1 - e_0 + e_1)}\right)\,.
    \end{aligned}
\end{equation} Since, $1 - e_1 + e_0, 1 - e_0 + e_1 \ge 1 - e_1 - e_0 > 0$ we have $\frac{1 - e_1 - e_0}{(1 - e_1 + e_0) (1 - e_0 + e_1)} > 0$ and we see that $a_1(x) \ge a_0(x)$ if and only if $\alpha_1(x) \ge \alpha_0(x)$. Now, noticing that (1) $P(Y = 1\mid X = x) \ge \nicefrac{1}{2}$ if and only if $a_1(x) \ge a_0(x)$, and (2) $Q(Y' = 1\mid X = x) \ge \nicefrac{1}{2}$ if and only if $\alpha_1(x) \ge \alpha_0(x)$ we have 
\[
\big\{x: Q(Y' = 1\mid X = x) \ge  \nicefrac{1}{2} \big\}  = \big\{x: P(Y = 1\mid X = x) \ge  \nicefrac{1}{2} \big\}\,.
\]

\end{proof}
